Examples for the standard conjecture of Hodge type

For each prime number $p$ and each integer $g \geqslant 5$, we construct infinitely many abelian varieties of dimension $g$ over $\overline{\mathbb{F}}_p$ satisfying the standard conjecture of Hodge type. The main tool is a recent theorem of Ancona on certain rank $2$ motives. These varieties are constructed explicitly through Honda-Tate theory. Moreover, they have Tate classes that are not generated by divisors nor liftable to characteristic zero. Also, we prove a result towards a classification of simple abelian varieties for which the result of Ancona can be applied to. Along the way, we prove results of independent interest about Honda-Tate theory and about multiplicative relations between algebraic integers.

==> packages.tex <==
%\usepackage[bbgreekl]{mathbbol}
\usepackage{amsthm,amsfonts,amssymb,amsmath,amsxtra}

%for having clickable links
\usepackage[hidelinks]{hyperref}

%?? Allows cref to distinguish between lemmas and theorems
\usepackage{thmtools}

% for better references
\usepackage{cleveref}


\usepackage[all]{xy}
% force xy arrow tips in computer modern font:
\SelectTips{cm}{}
\usepackage{tikz}
\usepackage{tikz-cd}
\usepackage{verbatim}


\usepackage[utf8]{inputenc} %pour que les accents soient bien compris

% \usepackage{pdfsync}
% \usepackage{showkeys}
\usepackage[a4paper, marginparwidth=60pt, margin=1.25in]{geometry}
\usepackage{mathrsfs}
\usepackage{marginnote}
\usepackage{stmaryrd}
\usepackage[english]{babel}
\usepackage{csquotes}

%to allow for nice mathbb 1:
\usepackage{dsfont}

%listings
\usepackage{listings}
%accents
\usepackage[T1]{fontenc} 
%Fancy letters
\usepackage[outline]{contour}
% for smart spacing after certain commands:
\RequirePackage{xspace}
% for programming features:
%\RequirePackage{etoolbox}
% for text environments which are automatically the natural width of the text they contain:
\RequirePackage{varwidth}
% for easy margin adjustment in enumerate and itemize environments:
\RequirePackage{enumitem}
% for good placement of super/subscripts to the left of symbols:
\RequirePackage{tensor}
% for various extensions of amsmath:
\RequirePackage{mathtools}
% allow tables to (if needed) split over multiple pages:
\RequirePackage{longtable}
% allow cells spanning multiple rows in tables:
\RequirePackage{multirow}
% allow nice line breaks inside cells (with \makecell{}):
\RequirePackage{makecell}
% for big integral signs:
\RequirePackage{bigints}
% for upward diagonal dots:
\RequirePackage{mathdots}
% for captions
\usepackage{capt-of}

% for local table of contents
%\usepackage{etoc}
%\usepackage{showlabels}
%stmary fonts [https://ctan.math.illinois.edu/fonts/stmaryrd/stmaryrd.pdf] :
%\usepackage{stmaryrd}
%fonts en plus

\usepackage[backend=bibtex, url = false, doi=false, isbn=false]{biblatex}

%fonts

%\usepackage[mtpbbi]{mtpro2}

%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "SHC_examples"
%%% End:

